Primitives for Contract-based Synchronization

We investigate how contracts can be used to regulate the interaction between processes. To do that, we study a variant of the concurrent constraints calculus presented in [1], featuring primitives for multi-party synchronization via contracts. We proceed in two directions. First, we exploit our primitives to model some contract-based interactions. Then, we discuss how several models for concurrency can be expressed through our primitives. In particular, we encode the pi-calculus and graph rewriting.

==> eptcsdata.tex <==
\providecommand{\firstpage}{67}
\providecommand{\publicationstatus}{Bliudze, Bruni, Grohmann, Silva (Eds.):\\Third Interaction and Concurrency Experience (ICE 2010)\\
EPTCS 38, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.38.8}{10.4204/EPTCS.38.8}}

